Automated Discovery Has No Universally Superior Harness

Autonomous discovery systems such as OpenEvolve and TTT-Discover are often used as general-purpose harnesses. However, in practice these are composite systems combining several design choices about archives, parent selection, exploration, and budget allocation into a single recipe. Because discovery runs are expensive and inherently stochastic, existing harnesses are often compared using too few independent trials to distinguish key methodological improvements from run-to-run variance. We systematically decompose OpenEvolve-style evolutionary search and the TTT-Discover search harness into its constituent components and systematically evaluate 30 budget-matched harnesses across 12 model-problem pairs using more than 3.1 million LLM rollouts and repeated-trial statistical analysis. Our results show that discovery harnesses have a generalization problem: No fixed harness is reliably superior across the evaluated model-problem pairs, and variants of OpenEvolve generally underperform simpler alternatives. Thus, harness choice is better viewed as a hyperparameter rather than as a universal recipe, and should be tailored to the specific problem and underlying model. We also find that early discovery progress predicts final performance, and use this property to present a budget-matched adaptive-allocation experiment that starts multiple harnesses, prunes weak partial runs, and reallocates compute to stronger survivors, outperforming both commitment to a randomly sampled fixed harness and a non-adaptive harness ensemble. Together, these results motivate shifting from fixed harness selection to online adaptation guided by early performance. We release all run pools including baseline null distributions for every model-problem pair as reusable statistical infrastructure against for future harness proposals.

==> figures/predictive_core_stats.tex <==
\begin{table}[t]
  \centering
  \caption{Predictiveness of early evolution progress. Spearman rank correlation is computed between the best score observed by a checkpoint and the final best score for the same run. Higher values mean the early ordering of runs better preserves the final ordering.}
  \label{tab:predictive_core_stats}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{llrrr}
    \hline
    Task & Model & Checkpoint fraction & Runs & Spearman early--final \\
    \hline
    Circle packing & Qwen2.5-3B-Instruct & 0.100 & 393 & 0.474 \\
    Circle packing & Qwen2.5-3B-Instruct & 0.250 & 393 & 0.662 \\
    Circle packing & Qwen2.5-3B-Instruct & 0.500 & 393 & 0.820 \\
    Circle packing & Qwen3-4B-Instruct & 0.100 & 289 & 0.279 \\
    Circle packing & Qwen3-4B-Instruct & 0.250 & 289 & 0.621 \\
    Circle packing & Qwen3-4B-Instruct & 0.500 & 289 & 0.868 \\
    Circle packing & GPT-OSS-20B & 0.100 & 162 & -0.002 \\
    Circle packing & GPT-OSS-20B & 0.250 & 162 & 0.348 \\
    Circle packing & GPT-OSS-20B & 0.500 & 162 & 0.732 \\
    Heilbronn triangle & Qwen2.5-3B-Instruct & 0.100 & 291 & 0.437 \\
    Heilbronn triangle & Qwen2.5-3B-Instruct & 0.250 & 291 & 0.773 \\
    Heilbronn triangle & Qwen2.5-3B-Instruct & 0.500 & 291 & 0.894 \\
    Heilbronn triangle & Qwen3-4B-Instruct & 0.100 & 343 & 0.146 \\
    Heilbronn triangle & Qwen3-4B-Instruct & 0.250 & 343 & 0.478 \\
    Heilbronn triangle & Qwen3-4B-Instruct & 0.500 & 343 & 0.762 \\
    Heilbronn triangle & GPT-OSS-20B & 0.100 & 196 & 0.259 \\
    Heilbronn triangle & GPT-OSS-20B & 0.250 & 196 & 0.530 \\
    Heilbronn triangle & GPT-OSS-20B & 0.500 & 196 & 0.784 \\
    \hline
  \end{tabular}%
  }
\end{table}


==> figures/strategy_deviation_mean_of_max.tex <==
\begin{table*}[t]
  \centering
  \caption{Budget-matched strategy-deviation evaluation. Each entry is the mean simulated final score over $10{,}000$ resampling trials under a five-full-run budget. Panel (a) reports fixed and single-stage strategies; panel (b) reports two-stage 25/50 schedules; and panel (c) reports three-stage 25/50/75 schedules. Schedule labels give the number of surviving configurations at successive stages. Bold indicates the best of all twelve strategies for that model--task pair.}
  \label{tab:ensemble_evolve_strategy_deviation}
  \scriptsize
  \setlength{\tabcolsep}{3.5pt}

  \textbf{(a) Fixed and single-stage strategies}\\[2pt]
  \begin{tabular}{llcccc}
    \hline
    Task & Model & Single config & Full portfolio & Single-stage 25\% & Single-stage 50\% \\
    \hline
    Circle packing & Qwen2.5-3B & 0.7594 & 0.7690 & 0.7896 & 0.7826 \\
    Circle packing & Qwen3-4B & 0.9027 & 0.9123 & 0.9245 & 0.9228 \\
    Circle packing & GPT-OSS-20B & 0.9788 & 0.9809 & 0.9816 & 0.9818 \\
    Heilbronn triangle & Qwen2.5-3B & 0.3044 & 0.2913 & \textbf{0.3566} & 0.3303 \\
    Heilbronn triangle & Qwen3-4B & 0.5230 & 0.5117 & 0.4411 & 0.4866 \\
    Heilbronn triangle & GPT-OSS-20B & 0.9423 & 0.9497 & 0.9455 & 0.9521 \\
    Second autocorrelation & Qwen2.5-3B & 0.9531 & 0.9536 & 0.9544 & 0.9545 \\
    Second autocorrelation & Qwen3-4B & 0.9582 & 0.9578 & 0.9596 & 0.9592 \\
    Second autocorrelation & GPT-OSS-20B & 0.9609 & 0.9618 & 0.9609 & 0.9620 \\
    \hline
  \end{tabular}

  \vspace{5pt}
  \textbf{(b) Two-stage schedules at 25/50\%}\\[2pt]
  \begin{tabular}{llccccc}
    \hline
    Task & Model & $10\!\to\!6\!\to\!2$ & $10\!\to\!4\!\to\!3$ & $9\!\to\!5\!\to\!3$ & $8\!\to\!6\!\to\!3$ & $7\!\to\!5\!\to\!4$ \\
    \hline
    Circle packing & Qwen2.5-3B & \textbf{0.7930} & 0.7896 & 0.7906 & 0.7879 & 0.7829 \\
    Circle packing & Qwen3-4B & \textbf{0.9252} & 0.9239 & 0.9223 & 0.9213 & 0.9182 \\
    Circle packing & GPT-OSS-20B & 0.9833 & 0.9828 & 0.9831 & 0.9826 & 0.9815 \\
    Heilbronn triangle & Qwen2.5-3B & 0.3395 & 0.3372 & 0.3317 & 0.3246 & 0.3146 \\
    Heilbronn triangle & Qwen3-4B & 0.5150 & 0.5097 & 0.5145 & 0.5167 & 0.5236 \\
    Heilbronn triangle & GPT-OSS-20B & 0.9585 & 0.9582 & 0.9585 & 0.9567 & 0.9556 \\
    Second autocorrelation & Qwen2.5-3B & 0.9550 & \textbf{0.9551} & 0.9550 & 0.9548 & 0.9546 \\
    Second autocorrelation & Qwen3-4B & 0.9601 & \textbf{0.9603} & 0.9600 & 0.9599 & 0.9593 \\
    Second autocorrelation & GPT-OSS-20B & 0.9634 & 0.9633 & \textbf{0.9635} & 0.9633 & 0.9629 \\
    \hline
  \end{tabular}

  \vspace{5pt}
  \textbf{(c) Three-stage schedules at 25/50/75\%}\\[2pt]
  \begin{tabular}{llccc}
    \hline
    Task & Model & $10\!\to\!5\!\to\!3\!\to\!2$ & $8\!\to\!5\!\to\!4\!\to\!3$ & $7\!\to\!6\!\to\!4\!\to\!3$ \\
    \hline
    Circle packing & Qwen2.5-3B & 0.7928 & 0.7876 & 0.7833 \\
    Circle packing & Qwen3-4B & 0.9250 & 0.9208 & 0.9191 \\
    Circle packing & GPT-OSS-20B & \textbf{0.9834} & 0.9825 & 0.9820 \\
    Heilbronn triangle & Qwen2.5-3B & 0.3418 & 0.3241 & 0.3161 \\
    Heilbronn triangle & Qwen3-4B & 0.5179 & 0.5283 & \textbf{0.5320} \\
    Heilbronn triangle & GPT-OSS-20B & \textbf{0.9594} & 0.9576 & 0.9560 \\
    Second autocorrelation & Qwen2.5-3B & \textbf{0.9551} & 0.9550 & 0.9548 \\
    Second autocorrelation & Qwen3-4B & \textbf{0.9603} & 0.9597 & 0.9596 \\
    Second autocorrelation & GPT-OSS-20B & 0.9634 & 0.9631 & 0.9629 \\
    \hline
  \end{tabular}
\end{table*}

